Differentiable PAC-Bayes Objectives with Partially Aggregated Neural Networks

We make three related contributions motivated by the challenge of training stochastic neural networks, particularly in a PAC-Bayesian setting: (1) we show how averaging over an ensemble of stochastic neural networks enables a new class of \emph{partially-aggregated} estimators; (2) we show that these lead to provably lower-variance gradient estimates for non-differentiable signed-output networks; (3) we reformulate a PAC-Bayesian bound for these networks to derive a directly optimisable, differentiable objective and a generalisation guarantee, without using a surrogate loss or loosening the bound. This bound is twice as tight as that of Letarte et al. (2019) on a similar network type. We show empirically that these innovations make training easier and lead to competitive guarantees.

==> our_files/preamble.tex <==
% Custom packages
\usepackage{amsmath}
\usepackage{amsthm}
\RequirePackage{mathptmx}  % replace the obselete times package in ICML style.
%\usepackage{unicode-math}  % must come after amsmath
\usepackage{multirow}
\usepackage{cleveref}
\usepackage{booktabs}
\usepackage{xcolor}

% Let align wrap around pages.
\allowdisplaybreaks

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}

% Custom Equation Commands
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\sign}{\text{sign}}
\newcommand{\Sym}{\text{Sym}}
\newcommand{\id}{\text{id}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\entropy}{\mathbb{H}}
\newcommand{\wq}{\tilde{q}}
\newcommand{\wQ}{\tilde{Q}}
\newcommand{\KL}[1]{\operatorname{KL}\left(#1\right)}
\newcommand{\D}[1]{\, \mathrm{d}#1}
\newcommand{\notw}{\neg\vec{w}}
\newcommand{\thetanotw}{\theta^{\boldsymbol{\neg}\vec{w}}}


% Command for often-repeated erf(...) final layer.
% \finallayer[<layer-no, default=2>]{<argument, e.g. α>}
\newcommand{\finallayer}[2][2]{\ensuremath{I\left(μ_{#1} \cdot ϕ(#2)\right)}}

\providecommand{\tightlist}{%
\setlength{\itemsep}{0pt}\setlength{\parskip}{0pt}}


% Probably remove this when submitting.
% just commenting is OK :)
\usepackage{xcolor}
\newcommand{\todo}[1]{\textbf{\textcolor{red}{TODO: #1}}}

